HiddenCut: Simple Data Augmentation for Natural Language Understanding with Better Generalization

Fine-tuning large pre-trained models with task-specific data has achieved great success in NLP. However, it has been demonstrated that the majority of information within the self-attention networks is redundant and not utilized effectively during the fine-tuning stage. This leads to inferior results when generalizing the obtained models to out-of-domain distributions. To this end, we propose a simple yet effective data augmentation technique, HiddenCut, to better regularize the model and encourage it to learn more generalizable features. Specifically, contiguous spans within the hidden space are dynamically and strategically dropped during training. Experiments show that our HiddenCut method outperforms the state-of-the-art augmentation methods on the GLUE benchmark, and consistently exhibits superior generalization performances on out-of-distribution and challenging counterexamples. We have publicly released our code at https://github.com/GT-SALT/HiddenCut.

==> vis.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{c|cccccc|c}
\hline
\textbf{Label }             & \multicolumn{6}{c|}{\textbf{Sentences from SST-2} }                                                                                                                               & \textbf{Set to be Cut}                                                                           \\  \hline \hline

N                  & {\cellcolor{blue3}a}                            & \cellcolor{blue0}sometimes                     & \cellcolor{blue5}tedious              & film                 & .                     &                       & tedious                                                                                 \\   %\cline{8-8}

N                  & \cellcolor{blue0}it's                         & \cellcolor{blue3} slow                          & --                   & \cellcolor{blue0} very                 & very                 & \cellcolor{blue3} slow                  & it's, slow, slow                                                                        \\ %\cline{8-8}

\multirow{2}{*}{N} & \cellcolor{blue0} the                          & film                          &  \cellcolor{blue3} suffers              & from                 & \cellcolor{blue0} a                    & \cellcolor{blue3} lack                  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}suffers, lack,   humor\end{tabular}}       \\
                   &  of                           &  \cellcolor{blue3}humor                         &                      &                      &                      &                       &                                                                                         \\ \hline \hline
\multirow{2}{*}{P} & \cellcolor{blue0} it's                         & a                             & \cellcolor{blue3} charming             & and                  & \cellcolor{blue0}  often                & \cellcolor{blue3} affecting             & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}it's, charming,  affecting\end{tabular}}  \\
                   & \multicolumn{1}{l}{journety} & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} &                                                                                         \\ % \cline{8-8}
P                  & a                            & \cellcolor{blue3} gorgeous                      & \cellcolor{blue3} high-spirited        & musical              & from                 & india                 & gorgeous,  high-spirited,                                                               \\ %\cline{8-8}
\multirow{2}{*}{P} & a                            & \cellcolor{blue5} delectable                    & \cellcolor{blue3} and                  & \cellcolor{blue3} intriguing           & theiller             & filled                & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}delectable, intriguing,  and\end{tabular}} \\
                   & \multicolumn{1}{l}{with}     & \multicolumn{1}{c}{\cellcolor{blue0}superises} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} &     \\ \hline                                                                                    
\end{tabular} \caption{Visualization of the attention weights in the last layer for constructing important set where HiddenCut would sample from. The sentences are from SST-2 labeled with negative(N) and positive(P). Deeper blue represents that those tokens receive higher attention weights. The set to be cut is defined by the top $\beta L$ words with higher attention weights. Here $\beta = 0.4$ and $L$ is the sentence length. 
\diyi{add or clarify highlighted tokens from baselines. Examples are not intuitive. visualize these examples on *out-of-distribution* - how many features, how much weights, before and after. }
%\diyi{this table helps a bit - "important set" is a bit less intuitive. change it to Set to be Cut? }
} \label{Tab:Vis}
\end{table*}




\begin{itemize}
    \item \textbf{DropBlock} \cite{Ghiasi2018DropBlockAR} randomly dropped spans in certain random hidden dimensions instead of the whole hidden space.
    
    \item \textbf{Random} HiddenCut  dropped the whole hidden representations of random spans of words.
    
    \item \textbf{LIME}  \cite{10.1145/2939672.2939778} \footnote{\url{https://github.com/marcotcr/lime}}: We utilized LIME on top of SVM classifier to pre-define the set of important words for HiddenCut to sample from. Note that the set was fixed across different layers during training.
    
    \item \textbf{GEM} \cite{yang-etal-2019-parameter} \footnote{\url{https://github.com/ziyi-yang/GEM}}: We applied the GEM algorithm \diyi{add a sentence or two to explain GEM, same to LIME, Gradient} to calculate and combine the novelty score, significance score ad uniqueness score based on hidden representations at every layer to generate the  set of important words. The scores and set would be updated during training.
    
    \item \textbf{Gradient} \cite{Yeh2019OnT}: We defined the set of important words by sorting their average absolute value of gradients in the backward-passing. The set would be updated during training.
    
    \item \textbf{Attention}: As described in Section~\ref{Sec:Strategy}, the importance was derived by the attention weights in self-attention layers. The set would also be updated during training.
    
\end{itemize}


